An Analysis of the Completion Time of the BB84 Protocol

The BB84 QKD protocol is based on the idea that the sender and the receiver can reconcile a certain fraction of the teleported qubits to detect eavesdropping or noise and decode the rest to use as a private key. Under the present hardware infrastructure, decoherence of quantum states poses a significant challenge to performing perfect or efficient teleportation, meaning that a teleportation-based protocol must be run multiple times to observe success. Thus, performance analyses of such protocols usually consider the completion time, i.e., the time until success, rather than the duration of a single attempt. Moreover, due to decoherence, the success of an attempt is in general dependent on the duration of individual phases of that attempt, as quantum states must wait in memory while the success or failure of a generation phase is communicated to the relevant parties. In this work, we do a performance analysis of the completion time of the BB84 protocol in a setting where the sender and the receiver are connected via a single quantum repeater and the only quantum channel between them does not see any adversarial attack. Assuming certain distributional forms for the generation and communication phases of teleportation, we provide a method to compute the MGF of the completion time and subsequently derive an estimate of the CDF and a bound on the tail probability. This result helps us gauge the (tail) behaviour of the completion time in terms of the parameters characterising the elementary phases of teleportation, without having to run the protocol multiple times. We also provide an efficient simulation scheme to generate the completion time, which relies on expressing the completion time in terms of aggregated teleportation times. We numerically compare our approach with a full-scale simulation and observe good agreement between them.

==> sections/applications.tex <==
\section{Performance Analysis of Elementary Communication Modules}\label{sec:app}

In this section, we apply the methods from Sect.~\ref{sec:rus} to derive the MGF of the completion times of certain communication modules and subsequently obtain their tail bounds/estimates.
%Recall that we use the notation $M_Z(t) = \mathsf{E}(e^{tZ})$ for a random variable $Z$.

We first consider an example where the success probability of the measurement event in a failure-prone procedure is independent of the latent variables, i.e., $p_{\theta}(\mathbf{L}_1) = p$.
Therefore, from~\eqref{eq:mgfW} we have: $W = \sum_{k=1}^N X_k$, where $N \sim \text{Geo}(p)$ and $X_k$'s are IID positive subexponential RVs with MGF $M_X$.
Thus,
$M_W(t)< \infty$ whenever $t < M_X^{-1}(\frac{1}{1-p})$.

\begin{example}\label{ex:1}
    Let us make further simplifications and
    assume $X = \max\{T_1,T_2\}$, where $T_1, T_2$ are IID $\text{Exp}(\lambda)$ and $X_k \sim X \thinspace \forall k$.
    That is, the \texttt{LOCC} duration is assumed to be negligible.
    Then
    $M_X(t) = 2 \lambda^2/((\lambda-t)(2 \lambda-t)).$
    Therefore, for $t<\lambda$, $M_X(t) < \frac{1}{1-p}$ implies:
    \begin{align*}
        t < \frac{\lambda(3-\sqrt{9-8p})}{2} = b' \thickspace \text{(Let)}~.
    \end{align*}
    %
    Applying~\eqref{eq:chernoffBound}, we have the following tail bound for $W$:
    %
    \begin{align}\label{eq:chernoffExample}
    \begin{aligned}
        \mathsf{P}(W \! > \! s) \!  &\le  \! \inf_{t \in [0,b')} \!  e^{-ts}\frac{p M_X(t)}{1 \! - \! (1 \! - \! p)M_X(t)} \\
        &= \! \inf_{t \in [0,b')}  \! e^{-ts} \frac{2 \lambda^2 p}{t^2 \! - \! 3\lambda t \! + \! 2 \lambda^2 p}~.
    \end{aligned}
    \end{align}
    %
    For $t \in [0,b')$, $e^{ts}(t^2-3\lambda t+2 \lambda^2 p)$ attains its supremum at
    $$t^*\!(s)\! = \! \max\!\bigg\{0,\frac{3 \lambda s\!-\!2\!-\!\sqrt{4\!+\!\lambda^2 s^2 (9\!-\!8p)}}{2s}\bigg\}~.$$
    
    Plugging into \eqref{eq:chernoffExample}, we have:
    \begin{align*} %\label{eq:optChernoffEx1}
        \mathsf{P}(W\!>\!s)\! \le e^{-t^*(s)s}\frac{2 \lambda^2 p}{(t^*\!(s))^2\!-\!3 \lambda t^*(s) \!+\! 2 \lambda^2 p}.
    \end{align*}
    Observe that $t^*(s) \to b'$ as $s \to \infty$ and $\mathsf{E}(X) = 3/2 \lambda.$
    This improves the best-known tail bound from~\cite{coopmans2022improved} for sufficiently large $s$, which has the exponential decay factor: $2p \lambda/3$.%<b'$ for $0<p<1$.
    
    To prove this claim, we consider the bounds in the logarithmic scale and show that the following sufficient condition holds for some $t<b'$ and for all sufficiently large $s$:
    \begin{align} \label{eq:condSharper}
      (t-\frac{2 p \lambda}{3})s > \log \mathsf{E}(e^{tW})-p~.  
    \end{align}
    
    Since $2 p \lambda/3<b'$ for $0<p<1$, we can pick $b'-\epsilon > 2 p \lambda/3$ which also satisfies $\mathsf{E}(e^{(b'-\epsilon)W})<\infty$.
    Thus, the condition~\eqref{eq:condSharper} is valid for $t = b'-\epsilon$ and for all $$s>\frac{\log \mathsf{E}(e^{(b'-\epsilon)W})-p}{b'-\epsilon-2 p \lambda/3}~.$$
    Clearly, this result can be extended to any positively distributed $X$.
    That is, under the assumption of $p_{\theta}(\mathbf{L}_1)\!=\!p$, the bound in~\eqref{eq:chernoffBound} is eventually sharper than the upper bound derived in~\cite[Prop. 2(c)]{coopmans2022improved} if $M_X\big(\frac{p}{\mathsf{E}(X)}\big)<\frac{1}{1-p}~.$ 
    Fig.~\ref{fig:chernoffEx1} presents a numerical comparison of these two bounds. \looseness = -1 \qed
\end{example}

Next, we consider an example where the success probability of the instantaneous event is dependent on the duration of constituent tasks.
%We also assume that the individual generation times follow exponential distribution.

\begin{example}[Diff-time cut-off]\label{ex:diffCO}

This example deals with the scenario where the two end nodes are joined by a single repeater.
To maintain the quality of the end-to-end link, an entanglement swap is performed at the repeater iff the difference between the individual completion times for link-level entanglement generation is within a threshold.
We seek to model the time until the entanglement swap at the repeater starts, which we denote by $W$.
Let us assume that the durations of the individual link generation attempts are distributed as $\text{SE}(\lambda, a)$ and so are the communication times heralding the success/failure of link generation.
Then, the completion times for both links are distributed as $T$, where
\begin{align*}
  M_T(t) &= \frac{e^{ta}\frac{\lambda}{\lambda-t} ~p e^{ta} \frac{\lambda}{\lambda-t}}{1-e^{ta}\frac{\lambda}{\lambda-t} (1-p) e^{ta}\frac{\lambda}{\lambda-t}} \\
  &= \frac{e^{2ta}\lambda^2}{(\lambda-t)^2-e^{2ta} (1-p)\lambda^2}~,
\end{align*}
$$$$
for all $t$ satisfying $(1-p)e^{2ta}(\frac{\lambda}{\lambda-t})^2<1$ and $t<\lambda$.

To compute the MGF of $W$ according to~\eqref{eq:mgfW}, we first note that $p_{\theta}(\mathbf{L}_1) = \mathbbm{1}_{|T_1-T_2|\le \tau}$ for some $\tau>0$, where $T_i$'s are the completion times for individual link generation and $T_i \sim T, i \in [2]$.
Next, we approximate $T-2a$ by a Gamma distribution.
The corresponding shape ($k'$) and scale ($\theta'$) parameter can be calculated using moment matching:
\begin{align}\label{eq:MoMdiffCO}
    k' \!&=\! \frac{2(a \lambda (1-p)+1)^2}{2(a \lambda (1\!-\!p)+1)^2-p (1\!-\!2 a^2 \lambda^2 (1\!-\!p))}, \nonumber \\
    \theta' \!&=\! \frac{2(a \lambda (1\!-\!p)+1)^2-p (1\!-\!2 a^2 \lambda^2 (1\!-\!p))}{ \lambda p (1-a  \lambda (1-p))}.
\end{align}
Since the completion times are observable to the repeater directly, we assume the corresponding communication time to be negligible.
Thus,
\begin{align}\label{eq:diffCoMgf}
    \expect{e^{tW}} &= \frac{\expect{e^{t\max\{T_1,T_2\}}\indicator{|T_1-T_2|\le \tau}}}{1-\expect{e^{t\max\{T_1,T_2\}}\indicator{|T_1-T_2|> \tau}}} \nonumber \\
    &= \frac{M^{(1)}(t)}{1-M^{(2}(t)} \thickspace \text{(Let)}~, 
\end{align}
for $t$ satisfying $M^{(2}(t)<1$.

Note that 
\begin{align*}
    &M^{(1)}(t) \\
    = & 2\! \int_{0}^\infty \!\!\!\int_{x}^{x+\tau} \!\!e^{t(y+2a)}\frac{y^{k'\!-1}e^{-\frac{y}{\theta'}}}{\Gamma(k') \theta'^{k'}} {\mathrm d y}\frac{x^{k'\!-1}e^{-\frac{y}{\theta'}}}{\Gamma(k') \theta'^{k'}} {\mathrm d x},
\end{align*}
and 
\begin{align*}
    &M^{(2)}(t) \\
    = & 2\! \int_{0}^\infty \!\!\!\! \int_{x+\tau}^\infty \!\!e^{t(y+2a)}\frac{y^{k'\!-1}e^{-\frac{y}{\theta'}}}{\Gamma(k') \theta'^{k'}} {\mathrm d y}\frac{x^{k'\!-1}e^{-\frac{y}{\theta'}}}{\Gamma(k') \theta'^{k'}} {\mathrm d x}.
\end{align*}
The Chernoff's bound (resp. Bahadur and Ranga Rao's estimate) can now be calculated using~\eqref{eq:chernoffBound} ( resp.~\eqref{eq:bahadurRaoSingleVar}),
as illustrated in Fig.~\ref{fig:gammaDiffCO}.
\qed 
\end{example}

==> sections/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{a1.png}}]{First A. Author} (M'76--SM'81--F'87) and all authors may include 
biographies. Biographies are often not included in conference-related
papers. This author became a Member (M) of IEEE in 1976, a Senior
Member (SM) in 1981, and a Fellow (F) in 1987. The first paragraph may
contain a place and/or date of birth (list place, then date). Next,
the author's educational background is listed. The degrees should be
listed with type of degree in what field, which institution, city,
state, and country, and year the degree was earned. The author's major
field of study should be lower-cased. 

The second paragraph uses the pronoun of the person (he or she) and not the 
author's last name. It lists military and work experience, including summer 
and fellowship jobs. Job titles are capitalized. The current job must have a 
location; previous positions may be listed 
without one. Information concerning previous publications may be included. 
Try not to list more than three books or published articles. The format for 
listing publishers of a book within the biography is: title of book 
(publisher name, year) similar to a reference. Current and previous research 
interests end the paragraph. The third paragraph begins with the author's 
title and last name (e.g., Dr.\ Smith, Prof.\ Jones, Mr.\ Kajor, Ms.\ Hunter). 
List any memberships in professional societies other than the IEEE. Finally, 
list any awards and work for IEEE committees and publications. If a 
photograph is provided, it should be of good quality, and 
professional-looking. Following are two examples of an author's biography.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{a1.png}}]{Second B. Author} was born in Greenwich Village, New York, NY, USA in 
1977. He received the B.S. and M.S. degrees in aerospace engineering from 
the University of Virginia, Charlottesville, in 2001 and the Ph.D. degree in 
mechanical engineering from Drexel University, Philadelphia, PA, in 2008.

From 2001 to 2004, he was a Research Assistant with the Princeton Plasma 
Physics Laboratory. Since 2009, he has been an Assistant Professor with the 
Mechanical Engineering Department, Texas A{\&}M University, College Station. 
He is the author of three books, more than 150 articles, and more than 70 
inventions. His research interests include high-pressure and high-density 
nonthermal plasma discharge processes and applications, microscale plasma 
discharges, discharges in liquids, spectroscopic diagnostics, plasma 
propulsion, and innovation plasma applications. He is an Associate Editor of 
the journal \emph{Earth, Moon, Planets}, and holds two patents. 

Dr. Author was a recipient of the International Association of Geomagnetism 
and Aeronomy Young Scientist Award for Excellence in 2008, and the IEEE 
Electromagnetic Compatibility Society Best Symposium Paper Award in 2011. 
\end{IEEEbiography}

